A fast radio burst cyclone in technicolour: evidence of plasma lensing

Fast radio bursts (FRBs) are bright, energetic, radio pulses of extragalactic origin. A dichotomy has emerged in the population: some produce repeat bursts, while the majority do not. Most repeating sources only show rare repetitions, and none have been studied extensively over the wide bandwidths necessary to disentangle the physical processes that produce emission from distortions to bursts caused by intervening ionised gas. Here we present radio observations of the most active repeating source, FRB 20240114A. Using an ultrawideband receiving system, we have detected 5526 repetitions, revealing an extreme spectral and temporal variability in the burst emission. The bursts exhibit longer-term broadband variations in central emission frequency over multiple months, and narrowband bursts that have correlations in central frequencies on time scales of milliseconds to minutes. The spectral and temporal properties are consistent with the source undergoing magnification by foreground plasma lenses, potentially embedded in a turbulent circumsource medium. This extreme example highlights the role of plasma lenses in the observed properties of burst emission and can explain the diversity in activity and energetics of the entire FRB population.

==> bib-macros.tex <==
\newcommand{\jan} {"Jan."}

\newcommand{\feb} {"Feb."}

\newcommand{\mar} {"Mar."}

\newcommand{\apr} {"Apr."}

\newcommand{\may} {"May"}

\newcommand{\jun} {"Jun."}

\newcommand{\jul} {"Jul."}

\newcommand{\aug} {"Aug."}

\newcommand{\sep} {"Sep."}

\newcommand{\oct} {"Oct."}

\newcommand{\nov} {"Nov."}

\newcommand{\dec} {"Dec."}

 %-------------------------------------------------------------------
 % Begin module:
 % \ProvidesFile{physjour.mbs}[2002/01/14 2.2 (PWD)]
\newcommand{\aa}{"Astron. \& Astrophys."}
\newcommand{\aasup}{"Astron. \& Astrophys. Suppl. Ser."}
\newcommand{\aj} {"Astron. J."}
\newcommand{\aph} {"Acta Phys."}
\newcommand{\advp} {"Adv. Phys."}
\newcommand{\ajp} {"Amer. J. Phys."}
\newcommand{\ajm} {"Amer. J. Math."}
\newcommand{\amsci} {"Amer. Sci."}
\newcommand{\anofd} {"Ann. Fluid Dyn."}
\newcommand{\am} {"Ann. Math."}
\newcommand{\ap} {"Ann. Phys. (NY)"}
\newcommand{\adp} {"Ann. Phys. (Leipzig)"}
\newcommand{\ao} {"Appl. Opt."}
\newcommand{\apl} {"Appl. Phys. Lett."}
\newcommand{\app} {"Astroparticle Phys."}
\newcommand{\apj} {"Astrophys. J."}
\newcommand{\apjsup} {"Astrophys. J. Suppl."}
\newcommand{\apss} {"Astrophys. Space Sci."}
\newcommand{\araa} {"Ann. Rev. Astron. Astrophys."}
\newcommand{\baas} {"Bull. Amer. Astron. Soc."}
\newcommand{\baps} {"Bull. Amer. Phys. Soc."}
\newcommand{\cmp} {"Comm. Math. Phys."}
\newcommand{\cpam} {"Commun. Pure Appl. Math."}
\newcommand{\cppcf} {"Comm. Plasma Phys. \& Controlled Fusion"}
\newcommand{\cpc} {"Comp. Phys. Comm."}
\newcommand{\cqg} {"Class. Quant. Grav."}
\newcommand{\cra} {"C. R. Acad. Sci. A"}
\newcommand{\fed} {"Fusion Eng. \& Design"}
\newcommand{\ft} {"Fusion Tech."}
\newcommand{\grg} {"Gen. Relativ. Gravit."}
\newcommand{\ieeens} {"IEEE Trans. Nucl. Sci."}
\newcommand{\ieeeps} {"IEEE Trans. Plasma Sci."}
\newcommand{\ijimw} {"Interntl. J. Infrared \& Millimeter Waves"}
\newcommand{\ip} {"Infrared Phys."}
\newcommand{\irp} {"Infrared Phys."}
\newcommand{\jap} {"J. Appl. Phys."}
\newcommand{\jasa} {"J. Acoust. Soc. America"}
\newcommand{\jcp} {"J. Comp. Phys."}
\newcommand{\jetp} {"Sov. Phys.--JETP"}
\newcommand{\jfe} {"J. Fusion Energy"}
\newcommand{\jfm} {"J. Fluid Mech."}
\newcommand{\jmp} {"J. Math. Phys."}
\newcommand{\jne} {"J. Nucl. Energy"}
\newcommand{\jnec} {"J. Nucl. Energy, C: Plasma Phys., Accelerators, Thermonucl. Res."}
\newcommand{\jnm} {"J. Nucl. Mat."}
\newcommand{\jpc} {"J. Phys. Chem."}
\newcommand{\jpp} {"J. Plasma Phys."}
\newcommand{\jpsj} {"J. Phys. Soc. Japan"}
\newcommand{\jsi} {"J. Sci. Instrum."}
\newcommand{\jvst} {"J. Vac. Sci. \& Tech."}
\newcommand{\nat} {"Nature"}
\newcommand{\nature} {"Nature"}
\newcommand{\nedf} {"Nucl. Eng. \& Design/Fusion"}
\newcommand{\nf} {"Nucl. Fusion"}
\newcommand{\nim} {"Nucl. Inst. \& Meth."}
\newcommand{\nimpr} {"Nucl. Inst. \& Meth. in Phys. Res."}
\newcommand{\np} {"Nucl. Phys."}
\newcommand{\npb} {"Nucl. Phys. B"}
\newcommand{\nt/f} {"Nucl. Tech./Fusion"}
\newcommand{\npbpc} {"Nucl. Phys. B (Proc. Suppl.)"}
\newcommand{\inc} {"Nuovo Cimento"}
\newcommand{\nc} {"Nuovo Cimento"}
\newcommand{\pf} {"Phys. Fluids"}
\newcommand{\pfa} {"Phys. Fluids A: Fluid Dyn."}
\newcommand{\pfb} {"Phys. Fluids B: Plasma Phys."}
\newcommand{\pl} {"Phys. Lett."}
\newcommand{\pla} {"Phys. Lett. A"}
\newcommand{\plb} {"Phys. Lett. B"}
\newcommand{\prep} {"Phys. Rep."}
\newcommand{\pnas} {"Proc. Nat. Acad. Sci. USA"}
\newcommand{\pp} {"Phys. Plasmas"}
\newcommand{\ppcf} {"Plasma Phys. \& Controlled Fusion"}
\newcommand{\phitrsl} {"Philos. Trans. Roy. Soc. London"}
\newcommand{\prl} {"Phys. Rev. Lett."}
\newcommand{\pr} {"Phys. Rev."}
\newcommand{\physrev} {"Phys. Rev."}
\newcommand{\pra} {"Phys. Rev. A"}
\newcommand{\prb} {"Phys. Rev. B"}
\newcommand{\prc} {"Phys. Rev. C"}
\newcommand{\prd} {"Phys. Rev. D"}
\newcommand{\pre} {"Phys. Rev. E"}
\newcommand{\ps} {"Phys. Scripta"}
\newcommand{\procrsl} {"Proc. Roy. Soc. London"}
\newcommand{\rmp} {"Rev. Mod. Phys."}
\newcommand{\rsi} {"Rev. Sci. Inst."}
\newcommand{\science} {"Science"}
\newcommand{\sciam} {"Sci. Am."}
\newcommand{\sam} {"Stud. Appl. Math."}
\newcommand{\sjpp} {"Sov. J. Plasma Phys."}
\newcommand{\spd} {"Sov. Phys.--Doklady"}
\newcommand{\sptp} {"Sov. Phys.--Tech. Phys."}
\newcommand{\spu} {"Sov. Phys.--Uspeki"}
\newcommand{\st} {"Sky and Telesc."}
 % End module: physjour.mbs
 %-------------------------------------------------------------------
 % Begin module:
 % \ProvidesFile{geojour.mbs}[2002/07/10 2.0h (PWD)]
\newcommand{\aisr} {"Adv. Space Res."}
\newcommand{\ag} {"Ann. Geophys."}
\newcommand{\anigeo} {"Ann. Geofis."}
\newcommand{\angl} {"Ann. Glaciol."}
\newcommand{\andmet} {"Ann. d. Meteor."}
\newcommand{\andgeo} {"Ann. d. Geophys."}
\newcommand{\andphy} {"Ann. Phys.-Paris"}
\newcommand{\afmgb} {"Arch. Meteor. Geophys. Bioklimatol."}
\newcommand{\atph} {"Atm\'osphera"}
\newcommand{\aao} {"Atmos. Ocean"}
\newcommand{\ass}{"Astrophys. Space Sci."}
\newcommand{\atenv} {"Atmos. Environ."}
\newcommand{\aujag} {"Aust. J. Agr. Res."}
\newcommand{\aumet} {"Aust. Meteorol. Mag."}
\newcommand{\blmet} {"Bound.-Lay. Meteorol."}
\newcommand{\bams} {"Bull. Amer. Meteorol. Soc."}
\newcommand{\cch} {"Clim. Change"}
\newcommand{\cdyn} {"Clim. Dynam."}
\newcommand{\cbul} {"Climatol. Bull."}
\newcommand{\cap} {"Contrib. Atmos. Phys."}
\newcommand{\dsr} {"Deep-Sea Res."}
\newcommand{\dhz} {"Dtsch. Hydrogr. Z."}
\newcommand{\dao} {"Dynam. Atmos. Oceans"}
\newcommand{\eco} {"Ecology"}
\newcommand{\empl}{"Earth, Moon and Planets"}
\newcommand{\envres} {"Environ. Res."}
\newcommand{\envst} {"Environ. Sci. Technol."}
\newcommand{\ecms} {"Estuarine Coastal Mar. Sci."}
\newcommand{\expa}{"Exper. Astron."}
\newcommand{\geoint} {"Geofis. Int."}
\newcommand{\geopub} {"Geofys. Publ."}
\newcommand{\geogeo} {"Geol. Geofiz."}
\newcommand{\gafd} {"Geophys. Astrophys. Fluid Dyn."}
\newcommand{\gfd} {"Geophys. Fluid Dyn."}
\newcommand{\geomag} {"Geophys. Mag."}
\newcommand{\georl} {"Geophys. Res. Lett."}
\newcommand{\grl} {"Geophys. Res. Lett."}
\newcommand{\ga} {"Geophysica"}
\newcommand{\gs} {"Geophysics"}
\newcommand{\ieeetap} {"IEEE Trans. Antenn. Propag."}
\newcommand{\ijawp} {"Int. J. Air Water Pollut."}
\newcommand{\ijc} {"Int. J. Climatol."}
\newcommand{\ijrs} {"Int. J. Remote Sens."}
\newcommand{\jam} {"J. Appl. Meteorol."}
\newcommand{\jaot} {"J. Atmos. Ocean. Technol."}
\newcommand{\jatp} {"J. Atmos. Terr. Phys."}
\newcommand{\jastp} {"J. Atmos. Solar-Terr. Phys."}
\newcommand{\jce} {"J. Climate"}
\newcommand{\jcam} {"J. Climate Appl. Meteor."}
\newcommand{\jcm} {"J. Climate Meteor."}
\newcommand{\jcy} {"J. Climatol."}
\newcommand{\jgr} {"J. Geophys. Res."}
\newcommand{\jga} {"J. Glaciol."}
\newcommand{\jh} {"J. Hydrol."}
\newcommand{\jmr} {"J. Mar. Res."}
\newcommand{\jmrj} {"J. Meteor. Res. Japan"}
\newcommand{\jm} {"J. Meteor."}
\newcommand{\jpo} {"J. Phys. Oceanogr."}
\newcommand{\jra} {"J. Rech. Atmos."}
\newcommand{\jaes} {"J. Aeronaut. Sci."}
\newcommand{\japca} {"J. Air Pollut. Control Assoc."}
\newcommand{\jas} {"J. Atmos. Sci."}
\newcommand{\jmts} {"J. Mar. Technol. Soc."}
\newcommand{\jmsj} {"J. Meteorol. Soc. Japan"}
\newcommand{\josj} {"J. Oceanogr. Soc. Japan"}
\newcommand{\jwm} {"J. Wea. Mod."}
\newcommand{\lao} {"Limnol. Oceanogr."}
\newcommand{\mwl} {"Mar. Wea. Log"}
\newcommand{\mau} {"Mausam"}
\newcommand{\meteor} {"``Meteor'' Forschungsergeb."}
\newcommand{\map} {"Meteorol. Atmos. Phys."}
\newcommand{\metmag} {"Meteor. Mag."}
\newcommand{\metmon} {"Meteor. Monogr."}
\newcommand{\metrun} {"Meteor. Rundsch."}
\newcommand{\metzeit} {"Meteor. Z."}
\newcommand{\metgid} {"Meteor. Gidrol."}
\newcommand{\mwr} {"Mon. Weather Rev."}
\newcommand{\nwd} {"Natl. Weather Dig."}
\newcommand{\nzjmfr} {"New Zeal. J. Mar. Freshwater Res."}
\newcommand{\npg} {"Nonlin. Proc. Geophys."}
\newcommand{\om} {"Oceanogr. Meteorol."}
\newcommand{\ocac} {"Oceanol. Acta"}
\newcommand{\oceanus} {"Oceanus"}
\newcommand{\paleoc} {"Paleoceanography"}
\newcommand{\pce} {"Phys. Chem. Earth"}
\newcommand{\pmg} {"Pap. Meteor. Geophys."}
\newcommand{\ppom} {"Pap. Phys. Oceanogr. Meteor."}
\newcommand{\physzeit} {"Phys. Z."}
\newcommand{\pps} {"Planet. Space Sci."}
\newcommand{\pss} {"Planet. Space Sci."}
\newcommand{\pag} {"Pure Appl. Geophys."}
\newcommand{\qjrms} {"Quart. J. Roy. Meteorol. Soc."}
\newcommand{\quatres} {"Quat. Res."}
\newcommand{\rsci} {"Radio Sci."}
\newcommand{\rse} {"Remote Sens. Environ."}
\newcommand{\rgeo} {"Rev. Geophys."}
\newcommand{\rgsp} {"Rev. Geophys. Space Phys."}
\newcommand{\rdgeo} {"Rev. Geofis."}
\newcommand{\revmeta} {"Rev. Meteorol."}
\newcommand{\sgp}{"Surveys in Geophys."}
\newcommand{\sp} {"Solar Phys."}
\newcommand{\ssr} {"Space Sci. Rev."}
\newcommand{\tellus} {"Tellus"}
\newcommand{\tac} {"Theor. Appl. Climatol."}
\newcommand{\tagu} {"Trans. Am. Geophys. Union (EOS)"}
\newcommand{\wrr} {"Water Resour. Res."}
\newcommand{\weather} {"Weather"}
\newcommand{\wafc} {"Weather Forecast."}
\newcommand{\ww} {"Weatherwise"}
\newcommand{\wmob} {"WMO Bull."}
\newcommand{\zeitmet} {"Z. Meteorol."}
 % End module: geojour.mbs
 %-------------------------------------------------------------------
 % Begin module:
 % \ProvidesFile{photjour.mbs}[1999/02/24 2.0b (PWD)]

\newcommand{\appopt} {"Appl. Opt."}
\newcommand{\bell} {"Bell Syst. Tech. J."}
\newcommand{\ell} {"Electron. Lett."}
\newcommand{\jasp} {"J. Appl. Spectr."}
\newcommand{\jqe} {"IEEE J. Quantum Electron."}
\newcommand{\jlwt} {"J. Lightwave Technol."}
\newcommand{\jmo} {"J. Mod. Opt."}
\newcommand{\josa} {"J. Opt. Soc. America"}
\newcommand{\josaa} {"J. Opt. Soc. Amer.~A"}
\newcommand{\josab} {"J. Opt. Soc. Amer.~B"}
\newcommand{\jdp} {"J. Phys. (Paris)"}
\newcommand{\oc} {"Opt. Commun."}
\newcommand{\ol} {"Opt. Lett."}
\newcommand{\phtl} {"IEEE Photon. Technol. Lett."}
\newcommand{\pspie} {"Proc. Soc. Photo-Opt. Instrum. Eng."}
\newcommand{\sse} {"Solid-State Electron."}
\newcommand{\sjot} {"Sov. J. Opt. Technol."}
\newcommand{\sjqe} {"Sov. J. Quantum Electron."}
\newcommand{\sleb} {"Sov. Phys.--Leb. Inst. Rep."}
\newcommand{\stph} {"Sov. Phys.--Techn. Phys."}
\newcommand{\stphl} {"Sov. Techn. Phys. Lett."}
\newcommand{\vr} {"Vision Res."}
\newcommand{\zph} {"Z. f. Physik"}
\newcommand{\zphb} {"Z. f. Physik~B"}
\newcommand{\zphd} {"Z. f. Physik~D"}

\newcommand{\CLEO} {"CLEO"}
\newcommand{\ASSL} {"Adv. Sol.-State Lasers"}
\newcommand{\OSA}  {"OSA"}
 % End module: photjour.mbs
%% Copyright 1994-2002 Patrick W Daly
\newcommand{\acmcs} {"ACM Comput. Surv."}

\newcommand{\acta} {"Acta Inf."}

\newcommand{\cacm} {"Commun. ACM"}

\newcommand{\ibmjrd} {"IBM J. Res. Dev."}

\newcommand{\ibmsj} {"IBM Syst.~J."}

\newcommand{\ieeese} {"IEEE Trans. Software Eng."}

\newcommand{\ieeetc} {"IEEE Trans. Comput."}

\newcommand{\ieeetcad}
 {"IEEE Trans. Comput. Aid. Des."}

\newcommand{\ipl} {"Inf. Process. Lett."}

\newcommand{\jacm} {"J.~ACM"}

\newcommand{\jcss} {"J.~Comput. Syst. Sci."}

\newcommand{\scp} {"Sci. Comput. Program."}

\newcommand{\sicomp} {"SIAM J. Comput."}

\newcommand{\tocs} {"ACM Trans. Comput. Syst."}

\newcommand{\tods} {"ACM Trans. Database Syst."}

\newcommand{\tog} {"ACM Trans. Graphic."}

\newcommand{\toms} {"ACM Trans. Math. Software"}

\newcommand{\toois} {"ACM Trans. Office Inf. Syst."}

\newcommand{\toplas} {"ACM Trans. Progr. Lang. Syst."}

\newcommand{\tcs} {"Theor. Comput. Sci."}
